Sonata: Query-Driven Network Telemetry

Operating networks depends on collecting and analyzing measurement data. Current technologies do not make it easy to do so, typically because they separate data collection (e.g., packet capture or flow monitoring) from analysis, producing either too much data to answer a general question or too little data to answer a detailed question. In this paper, we present Sonata, a network telemetry system that uses a uniform query interface to drive the joint collection and analysis of network traffic. Sonata takes the advantage of two emerging technologies---streaming analytics platforms and programmable network devices---to facilitate joint collection and analysis. Sonata allows operators to more directly express network traffic analysis tasks in terms of a high-level language. The underlying runtime partitions each query into a portion that runs on the switch and another that runs on the streaming analytics platform iteratively refines the query to efficiently capture only the traffic that pertains to the operator's query, and exploits sketches to reduce state in switches in exchange for more approximate results. Through an evaluation of a prototype implementation, we demonstrate that Sonata can support a wide range of network telemetry tasks with less state in the network, and lower data rates to streaming analytics systems, than current approaches can achieve.

==> background-old.tex <==
\section{Background}
\label{sec:background}

In this section, we discuss the basic requirements for a network telemetry system 
amidst recent advances in programmable data plane technologies and stream
processing frameworks for network monitoring. 

\subsection{Network Telemetry}
\label{ssec:back-tel}

As defined in~\cite{telemetry2016big}, ``Network Telemetry describes how information 
from various data sources can be collected using a set of automated communication 
processes and transmitted to one or more receiving equipment for analysis tasks. 
Analysis tasks may include event correlation, anomaly detection, performance monitoring, 
metric calculation, trend analysis, and other related processes." 



For the collection stage, network operators must grapple with how to
gather information from a distributed set of collectors to some
centralized location.  Typically, operators employ tools that transform the
data at the distributed collectors to some aggregated statistical values (e.g.,
per-link counters) and then use fixed protocols (\eg~SNMP) for central
collection. Alternatively, tools can locally reduce the data to a randomly
sampled subset of the original data and again use fixed protocols (\eg~NetFlow,
IPFIX, etc.) for central collection. While these tools succeed in
decreasing the volume of the data that is transferred for
analysis, the loss of information due to such data reductions is, in general, too
severe and prevents any meaningful real-time decision-making based on the
collected data.~\footnote{Note that the definition of {\em real-time} is
different for different networks. In wide-area settings where high latency
values dominate, it is reasonable to consider detecting events within a few
seconds as real-time. This is different for data center networks where detection
within a few milliseconds is considered as real-time.} 

For the analysis stage, network operators have typically relied on protocol-specific tools  
such as~XX~\cite{}. However, ``scaling out" these tools and platforms to support the 
analysis of the high-volume and high-velocity data at packet-level granularity that 
effective real-time decision-making demands is non-trivial and poses fundamental 
challenges. As a result, most of the currently deployed network telemetry systems 
are not able to detect and/or act on network events of interest in real-time.

\subsection{Scalable Stream Processors}
\label{ssec:back-stream}
Stream processors use a simple programming model, {\em Dataflow}, which operates on a
continuous stream of tuples using successive applications of deterministic transformations.
A {\em Dataflow} query is a sequence of such transformations over a stream of tuples. 

Network operators can express their monitoring queries as a pipeline of transformations 
using the functional APIs provided by these stream processors. While expressing monitoring
queries using such functional APIs allows for seamless scaling of the analysis stage, the
{\em Dataflow} programming model can only be applied on general-purpose compute
nodes. As a result, network operators must still use different frameworks for
performing the collection, transformation, and transportation of raw packet
streams into tuples before the stream processors can be employed for further
analysis. It is thus still the network operator’s responsibility to manually
stitch the two frameworks together---a task that makes this setup brittle, prone
to failures, and with a steep learning curve. 

Note that we do not consider point solutions in the design space where the collection stage 
consists of simply collecting all the raw packets from the network and relying on the linear 
scalability property of state-of-the-art stream processors; that is, applying 
{\em dataflow} queries over all the raw packets. While ``scaling out” 
the collection stage is possible~\footnote{There are commercial products
capable of performing lossless packet capture at link speeds of 100 Gbps and
beyond~\cite{niksun}.}, ``scaling out” the analysis stage has its limits. Even
though modern stream processing platforms are designed to scale linearly, the
cost and complexity of processing hundreds of millions of packet tuples for a
single query is simply too high to work in practice~\cite{osoc-scale}. 

Currently considered frameworks such as {\em streaming (network)
telemetry}~\cite{google-nt, cisco-nt, sflow-nt, arista-nt} are
early, industry-led efforts towards providing more granular, real-time 
information about the network, but they still fall far short of the type of
packet-level network telemetry systems we envision.

\subsection{Programmable Dataplane}
\label{ssec:back-pisa}
\begin{figure}[t!] \centering \includegraphics[trim={0 69pt 0
125pt},clip,width=\linewidth]{figures/pisa.eps} \caption
{Protocol Independent
Switch Architecture.\label{fig:pisa}}
\end{figure}

Historically, the use of fixed protocols for transforming raw data packets in
the network before the analysis stage prevented network operators from
expressing queries that maintain custom state or custom packet processing logic.
 These limitations naturally imposed a division between the frameworks
 employed for the collection and analysis stages. In contrast, recently proposed
 {\em Protocol Independent Switch Architecture (PISA)} switches (see Figure~\ref
 {fig:pisa}) provide many features that permit the implementation of customized
 packet processing and state management logic in the data plane~\cite{rmt,
 p4-xilinx, barefoot-blog, P4, p4-netronome}. {\em In-band Network Telemetry 
 (INT)}~\cite{INT} is a recent example framework employing PISA targetd that
 allows the collection and reporting of network state by the data plane without
 requiring intervention or work by the control plane. Importantly, by
 supporting the execution of a subset of {\em dataflow} operations in the
 data plane itself, PISA features permit the critical integration of the
 collection and analysis stages. In the following, we list specific features of
 PISA targets that enable the execution of arbitrary {\em dataflow} operators
 in the data plane.

\smartparagraph{Programmable Parsing}.  PISA targets allow for the specification of new packet 
header formats for parsing and deparsing packets.  Programmable parsing enables both the 
extraction of desired packet header fields for answering arbitrary queries and the definition 
of application-specific header formats for sending streams of tuples to a stream processor.

\smartparagraph{State Management Primitives.} Operators will write queries that apply
{\em Dataflow} operators over packet header fields, but they may also require
per-packet state or calculations for other dataflow operations. Such fields are
easily implemented in user-defined metadata. Additionally, these queries often require state 
across sequences of packets (\eg a sum is calculated across a sequence of packets by 
applying the {\tt reduce} operation \rjh{forward-reference without the table from commit
4043fe36f38a25e2d70466933df20b1d3fb81695.  I say we bring it back into the
section.}). Both these requirements can be easily accommodated in modern PISA
switches. 

\smartparagraph{User-defined Hashing.} Operators like {\tt reduce} and {\tt distinct} require 
maintaining state in the data plane depending on combinations of {\em query-specific} 
reduction keys. Support for hash calculations over query-defined field combinations enable 
these operators to maintain the required state in the data plane.

\smartparagraph{Flexible Match/Action Table Pipelines.} Flexible match action tables in the 
reconfigurable data plane ensure that novel combinations of {\em Dataflow} operators 
can be applied to the right subsets of matched packets.

The observed rapid advances in programmable data plane technologies and constant 
innovations in stream processing argue strongly in favor of designing \system in a strictly 
modular fashion so that it can accommodate different network operators with different 
configurations at their disposal. For example, if provided with a data plane that
has less flexible features, \system's runtime should be aware of and adapt to
the available feature set. Whatever queries cannot be implemented in the given
data plane will be offloaded to the stream processor, but such offloading can be
expected to have scalability implications.






==> discussion.tex <==
\section{Future Directions}\label{sec:discussion}
\ag{TBD}

%In contrast to existing programmable data planes which are relatively
%fixed-function (\eg, OpenFlow chipsets), emerging technologies, such as
%those that enable in-band network telemetry via
%P4~\cite{bosshart2014p4}, make it possible to redefine packet-processing
%control-flow at compile time. This capability may enable a variety of
%richer measurement applications that could take advantage of a
%programmable, stateful network data plane.
%
%One example of such an application could be to use in-band network
%telemetry to attach latency statistics to packets as they travel through
%network devices, thus making it possible to pinpoint sources of
%increased latency, packet loss, or congestion.  The network devices
%could affix {\em additional} data to packet headers (\eg, latency at
%each hop, the set of switches that the packet traversed) which could
%subsequently be used as input to a tuple-based query.  Another such
%example is the use of so-called ``active'' machine learning algorithms
%that improve their accuracy over time by requesting more examples of
%labeled data. These algorithms could potentially use iterative
%refinement to define a query that asks for more examples of attack
%payloads when the algorithm needs to improve its accuracy.
%
%Moving forward, \system could drive real-time control decisions. 
%The output of \system queries could serve as an input to inference
%algorithms which could then drive the installation not only of
%forwarding table rules to refine the measurements, but also of
%forwarding table rules that affect how traffic is forwarded.  
%Support for approximate
%queries (\eg,~\cite{motwani2002query,cormode2008approximate}) that can
%operate on samples of network traffic is another interesting avenue for
%future work.  In many cases, even an approximate result could reveal the
%existence of an attack or performance degradation



==> future.tex <==
\section{Future Work}\label{sec:future}
%1. Multiple queries: we already allude to this in section 4.3.3 but could expand slightly on the promise of potentially significant additional benefits in cost savings (reduction in wasted resources) due to the selection of query plans that excel in identifying and benefitting from shared resources among a given set of parallel running queries.
%
%2. Active learning: again, we already alluded to this in section ? but since  Nick likes this topic, we may want to expand on this as well, maybe all the way to suggesting theuse of Sonata itself to how to learn what at what time …
%
Currently, our prototype is limited to a single monitoring switch.  We envision future versions of \system where an enhanced runtime partitions queries among sets of switches in a distributed context.  We also envision a future where clusters of quasi-autonomous instances of \system coordinate to achieve optimal query execution.
% Distributed setting: this is probably the item we should and could comment on in most  detail, connecting it to the existing efforts on geo-distributed or wide-area analytics (sprinkling in a few references you already have), describing the option of having a version of Sonata running in each remote node and also in the central node, and mentioning how this would enrich query partitioning by having the options to partition differently across remote nodes and also running parts centrally while the rest remotely.

==> implementation.tex <==
\section{Implementation}
\label{sec:drivers}

Our prototype is implemented in {Python} (around 9,000 lines of code). We use 
P4 Behavioral Model (bmv2) PISA switch, and Open vSwitch 2.5 as data plane
targets as well as Spark 1.6.1 as our streaming target. We will now describe
how we implement the runtime system and the data plane drivers.



\subsection{Find Optimal Query Plans: Runtime}
\label{ssec:runtime}
We will now describe how runtime selects the right exectuion plan for each
query. 
%Runtime's primary task is to learn the right execution plan for each input
%queries. We will now describe how it selects the execution plan for e
%For that, it first uses the input query and the APIs exposed by the
%target's drivers as shown in Table~\ref{tab:driver-api} to build the query plan
%graphs. It then generates queries for each node in the graph and then uses
%training data collected periodically from the network to estimate the weights
%for the query plan graphs. It then feeds these weighted query plan graphs to the
%learning module to learn the right execution plan for each query. It then sends
%the partitioned queries to the respective drivers. 

\begin{table}[t]
\begin{footnotesize}
\begin{tabular} {| m{.65 in} m{2.1in} |}
\hline
{\bf Driver API} & {\bf Description} \\ \hline
{\tt {\bf isSupported}(q)} & Returns whether the target can execute query {\tt q}.\\
{\tt {\bf getCost}(q,t)} & Returns normalized cost of executing query {\tt q} over 
the target, given training data {\tt t}. \\ 
{\tt {\bf compile}([q])} & Executes list of queries [{\tt q}] over the target.\\
\hline
\end{tabular}
\end{footnotesize}
\caption{Target-specific driver's API exposed to \system's runtime.}
\label{tab:driver-api} 
\end{table}

\smartparagraph{Building the Query Plan Graphs.}
Runtime first builds query plan graph for each query. It first enumerates the set of 
partitioning plans ($\mathcal{P}$) for a given
query, ($q$). It  generates incrementally more complex partitioned
sub-queries by adding one operator from the orginal query at a time. For
each partitioned query, it calls the {\tt isSupported}() function (see
Table~\ref{tab:driver-api}), exposed by target's driver. This function reports
whether or not the target can support the generated sub-query and parse the
fields required for the operation.

%\smartparagraph{Enumerating Refinement Plans.}
To enumerate the set of refinement levels $R$ for a given query, \system's runtime 
first determines the set of refinement keys that can be used for iterative
refinement. They are determined by identifying the set of fields that (1)~are
used as keys in stateful dataflow operations like {\tt reduce} and {\tt
distinct} and (2)~have a hierarchical structure so as to be replaceable by
their coarser versions without missing any traffic that satisfies the original
query. 
%While it is possible to have more than one candidate field for iterative
%refinement, it is also possible to not find any candidate for refinement for a
%query. Consider the example of the query for detecting sidejacking attacks 
%(see table~\ref{tab:apps}). This query cannot benefit from iterative refinement
%because the two fields {\tt sessionID} and {\tt userAgent} that are used in the 
%{\tt distinct} operation do not have any hierarchical structure. 

After identifying the refinement keys, the runtime enumerates the refinement
levels using pre-configured field-specific levels. For example,
header fields like {\tt dstIP}, {\tt srcIP} etc. can naturally be refined at the 
granularity of one bit, resulting in a maximum of 32 potential refinement levels
for these fields that conform to the IPv4 address format.  
%One could imagine
%only considering $n$, $k$-bit intervals over the 32 possible maximum, but giving
%\system all the refinement levels possible allows it to learn the best sequence
%of refinement levels. 
Other fields like {\tt dns.qname} can be similarly
refined at the granularity of sub-domain levels. Finally, the runtime uses
enumerated sets $R$, $\mathcal{P}$, and $L$ to generate the nodes and the edges
for the query plan graphs. 

\smartparagraph{Estimating Weights for Query Plan Graph.}
In order to compute the weights for each edge in the query plan graph, runtime
needs to generate queries for each node in the graph. It adds {\tt map} operation
to execute queries at coarser level as shown in Figure~\ref{fig:ir}. However, selecting
the appropriate threshold at coarser levels is challenging. For example, in 
Query ~\ref{asymm-query},
the network operator specifies a threshold value on line 7 for a specific {\tt
dstIP} (also written as {\tt dIP/32}).  However, at coarser refinement levels,
~\eg~{\tt dstIP/8}, it would be inappropriate to apply the same threshold as
originally specified because the field in question is now an aggregate count
bucket and not a specific {\tt dstIP/32}. \system's runtime has to select
appropriate thresholds for each node in the graph such that no traffic that
satisfies the query at the finest level is missed.  
%high-level query both to filter out the uninteresting traffic from the coarser levels of refinement and also
%select an appropriate threshold value that adjusts for the less granular data
%observed at coarser refinement levels. 
%use training data to learn the weights for the edges in the query
%plan graph, the runtime must first create concrete implementations of the
%original high-level \system query at each node in the query plan graph.  The
%runtime must generate these concrete implementations for both the streaming and
%data plane targets, according to that node's partition plan. 

%Naive solutions to the threshold selection problem could eliminate
%the benefits of using iterative refinement altogether; therefore, our
%solution to this problem relies on using representative training data to let the
%runtime select appropriate threshold values for each refinement level. 
To address this challenge, the runtime first runs the query at the finest 
refinement level over the training data to identify the portion of traffic that satisfies 
the original input query. It then backtracks to a coarser refinement level, runs the 
query again, but this time tracks the results for aggregate count buckets that contain 
the results at the next finer refinement level---selecting the minimum 
count, of all count buckets, as the threshold value for this coarser refinement level.  
It continues this process until it reaches the coarsest refinement level thereby ensuring that
at each refinement level, it selects a threshold greater than or equal to the
original threshold without missing any traffic that satisfies the query. 

After generating queries for each node, runtime joins queries for pair of nodes---ensuring
that the query at finer level is only applied of traffic that satisfies the query
at the coarser level. It then provides the training data, and joined query for each
node as input to driver's {\tt getCost} (see Table~\ref{tab:driver-api}) to compute weight.


%a concrete implementation of corresponding data plane and
%streaming target queries for each node in the query plan graph, the runtime
%provides the training data and the queries for the pair of nodes on each edge in
%the graph as input to the {\tt getCost} (see Table~\ref{tab:driver-api})
%function exposed by the targets' drivers. This function estimates the number of
%bits required to execute the partitioned query in the data plane and the number
%of tuples to be processed by the streaming target. The runtime uses this
%information to update weights for the query plan graph edges. 

After translating the training data into a weighted query plan graph, the
runtime applies the learning algorithm to select query plan. It then calls
each target-specific driver's {\tt compile} function, as described in Table~\ref
{tab:driver-api}, for executing refined and partitioned queries over the respective
targets. We will now describe how these drivers execute the partitioned queries.



%\begin{table}
%\noindent\begin{minipage}{\columnwidth}
%\lstset{belowskip=0pt}
%\begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
%caption= P4 code showing how partitioned Query~\ref{asymm-query} 
%is executed over PISA targets, 
%captionpos=b, label=dp-queries, 
%basicstyle=\footnotesize, 
%numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
%action update-metadata(){
% modify_field(meta.qid, qid);
% modify_field(meta.drop, 0); 
% ...}
%action update-output-headers(){
% add_header(out_header);
% modify_field(out_header.qid, meta.qid); 
% ...}
%control ingress {
% apply(update-metadata);
% apply(filter_1);
% ...
% if (meta.drop == 0) {
%  apply(report_packet);}}
%control egress {
% apply(update-output-headers);}
%\end{lstlisting}
%\lstset{aboveskip=\medskipamount}
%\end{minipage}
%\end{table}
%\noindent

\subsection{Compiling Dataflow Queries: Drivers}
\label{ssec:drivers}
Since streaming targets already implement all of \system's dataflow operators,
compiling partitioned queries over streaming targets is trivial. Thus, in this
section, we will primarily focus on how \system compiles partitioned queries
over the data plane targets. 
%We first describe how it stitches together
%primitives for individual operators to configure a packet processing pipeline
%for a single query in the data plane. We then present how it combines these
%pipelines together to execute multiple queries inthe data plane. 

\smartparagraph{Compiling A Single Query.}
To compile a dataflow query over PISA targets, we first configure match/action
tables and hash tables required to execute individual operators for the query as discussed
in Section~\ref{sec:scale}. 
We then configure these operator-specific tables to ensure that they are applied
in sequence. We take two goals into consideration while compiling dataflow queries 
for PISA targets: (1)~the packet processing pipelines should not affect a packet's 
forwarding behavior~\ie, transformations over a packet's header should not be
applied over the packet's actual header fields; (2)~the mirroring overhead for
each query should be minimal~\ie, we should only mirror packets that need to be
reported to the streaming target. To achieve the first goal,  we create
query-specific metadata fields---copying information from the original header
fields to these fields. To achieve the second goal, we maintain additional one
bit metadata field,~{\tt report}, for each packet that specifies whether or not
the result associated with the packet should be reported to the streaming
target.
%At the end of the query, if the {\tt report} field is set, then 
%the packet is cloned and reported to the streaming target preserving the original packet to
%continue being processed through logic to determine its forwarding behavior.

\smartparagraph{Compiling Multiple Queries.}
Most streaming systems execute multiple queries in parallel, where each query
operates over its own copy of the input stream. Replicating this
paradigm in the data plane would require us to clone a packet copy for
each query.  However, naively creating copies of packets for each query in the
data plane is too expensive for any practical deployment, especially in
high-volume networks. In practice, a packet is unlikely to satisfy the filters
for all queries. Thus, a solution with less overhead could clone the packets
after all queries' filter operators have been applied. However, even if a packet
satisfies as few as two queries, the cloning overhead of this alternative
method is as high as 100\% which is prohibitive for most production networks.

To solve this problem, we execute queries at the data plane sequentially.  Now,
we cannot make the decision whether or not to report a packet to the stream
processor at the conclusion of a single query's operators.  Instead, we take the
union of the {\tt report} bit for each query. After all queries have been
evaluated for a given packet, the data plane simply makes a single copy for
delivery to the stream processor, if required. This design choice significantly
reduces the mirroring overhead and requires only an additional bit of state.
However, when reporting data to the stream processor, this approach requires the
single packet to carry the metadata fields for all reported queries---limiting
the number of queries we can support on a single switch. Additionally, our
current implementation configures a separate match/action table for each
operator. For some PISA targets, the number of match/action tables we can
configure are limited. This problem can be addressed by sharing resources
between multiple queries. We leave this exploration for future work. 

\smartparagraph{Stitching Data Plane \& Streaming Targets.}
In our prototype, we employ a span port that connects the monitoring switch
and the stream processor.  When a switch detects that a given packet must be
reported to the stream processor, we first modify the mirrored packet to only 
include the fields to be reported to the streaming target.  We also truncate all
reported packets to a minimum size unless the streaming target needs to apply 
operations over the packet's payload.  This ensures that the packet parser has 
fewer bits to parse.
The data plane driver configures a packet parser to decode packets received over
the span port. The packet parser uses {\tt scapy}~\cite{scapy} to extract the
values from the raw packets. The decoded packets are then sent as tuples to the
streaming target for further processing. A streaming target receives tuples
containing all of the desired fields and an identifier establishing to which
query this tuple belongs.


\smartparagraph{Updating Query Executions.}
%\label{ssec:updates}
At the end of every window interval, a given query's output is computed by the
streaming target, which it sends to the runtime system. At the end of every
window interval, a query's execution plan may proceed to the next refinement
level. The runtime system processes the output and updates any {\tt filter}
operations for partitioned queries~\ie~to support a finer refinement level. It
then calls the {\tt compile} function to update the packet processing pipeline
in the data plane. The data plane driver updates the respective match/action
table entries as well as resets the values of stateful variables for each query.
%
%These factors contribute to how quickly the query executions are updated for
%each window interval. Our goal is to keep this delay as low as possible, as
%higher delays will result in reporting incorrect statistics for query outputs.
%Most of these contributing factors can be addressed by appropriate resource
%provisioning at the streaming targets, and efficient implementations for
%handling the output at runtime and the data plane drivers. Updating the data
%plane tables and registers, however, is the most time consuming step. We
%quantify these overheads in Section~\ref{sec:eval} and hypothesize they are due
%the inefficient nature of the P4 software switch.


==> intro-old.tex <==
\section{Introduction} \label{sec:intro}
The demands on operators to keep modern networks running are unrelenting.
At unpredictable intervals, networks perform poorly or suffer downtime due 
to high usage, failures, configuration errors, or attacks from malicious parties. 
Downtime and security breaches can not only lead to significant financial losses for
enterprises, ISPs and content providers~\cite{downtime}, but can also be
expected to pose serious public safety risks for tomorrow's ``smart'' homes and
cities using IoT devices. 

To cope with these realities, network operators have started to leverage
{\em network telemetry} frameworks~\cite{NT-ieft16}w in which information 
from various data sources within the network is collected using a set of
automated communication processes and transmitted to one or more pieces of
receiving equipment for conducting analysis tasks. These tasks include queries
for event correlation, anomaly detection, performance monitoring, metric
calculation, trend analysis, and other processes aimed at mining and learning
from the collected data and assist network operators in detecting 
security and performance degradations in a real-time fashion.~\cite
{NT-ieft16}~\footnote {Definition of {\em real-time} is
different for different networks. It is reasonable to consider a few seconds as
real-time in wide area settings and a few milliseconds as real-time in data
center networks.} A key characteristic of traditional network telemetry systems
is their rigid division of labor into two separate stages, namely the data 
{\em collection} and data {\em analysis} stages, and this division has naturally
led to the development of separate toolchains for performing each stage.

\smartparagraph{Collection Stage.} Different queries require input data at different
levels of granularity. Efficiently answering those queries often forces network 
operators to grapple with the {\em too much vs.
too little} conundrum: collecting too much information, like full packet
captures, provides all the information required for the analysis stage but is
hard to scale; collecting too little information, \ie~using tools that perform
fixed transformations such as sampling over the raw packets can scale but often 
provides insufficient details for effective analysis. Thus, for each query,
network operators typically need to reason about {\em what} to collect, and at 
what level of granularity (flow, packet, etc.).  To add to the operators’ burden,
they then have to instrument the myriad collection tools (e.g., 
NetFlow~\cite{netflow}, sFlow~\cite{sflow}, SNMP~\cite{snmp}, or raw 
packet captures~\cite{pcap}) to support their choices---often having to configure
these collection tools using platform-specific, and low-level APIs. 

\smartparagraph{Analysis Stage.} After successful collection, network operators use 
or mine their data by applying different analysis tools that often depend on the 
format of the collect data. For example, the same tool that analyzes raw packet 
captures typically cannot be applied over SNMP data. Moreover, for data collected 
at fine levels of granularity (\eg~packet-level), scaling the analysis while also
ensuring the required real-time response capabilities is non-trivial. In fact, under 
this real-time constraint, the analysis stage is confined to performing {\em streaming 
analytics}; that is, a single pass over the continuous stream of collected data 
is all that can be afforded for analysis. On the one hand, network operators have
embraced recent advances in the area of scalable stream processing~\cite
{opensoc, spark, flink, tigon, gigascope} where analysis queries are expressed 
as a sequence of {\em dataflow} operators. At the same time, systems like 
OpenSOC~\cite{opensoc} that already leverage stream processing for network analysis
are restricted in terms of their scalability mainly because of the high bandwidth 
demand that results from its hard-wired design choice of collecting all raw packets 
for analysis. Worse yet, even though these latest stream processor solutions are 
designed to scale linearly, the cost and complexity of processing all the collected 
raw packets are prohibitively high~\cite{osoc-scale} in production networks with 
traffic rates in the multi-tbsp range. 

These initial advances in streaming analytics notwithstanding, progress towards
a principled approach to coupling rather than separating the collection and 
analysis stages of (packet-level) network telemetry so that they can inform 
one another has been slow. As a result, today’s network telemetry systems continue
to be plagued by major mismatches between the data that is collected and the data 
is needed for analysis, severe limitations to the systems’ ability to react in 
real-time to new network events, and a largely piecemeal approach to the writing 
of collection- and analysis-specific queries and resulting tool chains. In fact,
operators are still often forced to write custom glue code that manually stitches 
together the various collection output formats to answer a single high-level query
about the state of the network. At the same time, any changes to the {\em how},
{\em where} or {\em what} at the data collection stage can trigger changes for 
the analysis stage that may require a complete or partial overhaul of the existing
analysis queries. The combination of these features results in a workflow for today's
network telemetry systems that is brittle, error-prone and difficult to maintain.

\smartparagraph{\system.} In this paper, we present a new packet-level telemetry system
\system\footnote{Scalable Streaming Network Traffic Analysis (SNTA, or 
``SONATA"’).} that provides network operators with a single query interface that
allows them to express monitoring queries in a familiar programming paradigm; 
that is, as a sequence of {\em dataflow} operators applied directly over the raw 
packet stream where packets are modeled as a collection of arbitrary (unstructured)
fields. This abstraction makes it easier for network operators to express a wide 
range of network telemetry queries. Rather than manually stitching together 
disparate formats and tools from underlying collection platforms' APIs, \system
presents a single query interface in which operators can express high-level queries 
without having to worry about the details of how the execution of these queries is 
scaled. In effect, \system does away with the conventional division of network telemetry 
into separate {\em collection} and {\em analysis} stages and provides explicit 
mechanisms for the two stages to inform one another so as to ``orchestrate" the best 
way to execute the expressed monitoring queries.

To enable this orchestration and effectively scale the execution of telemetry 
queries expressed at packet-level granularity, we make two domain-specific observations. 
First, we observe that recent advances in the area of {\em Protocol 
Independent Switch Architectures (PISA)}~\cite{rmt, p4-xilinx, barefoot-blog, 
P4, p4-netronome} have made it possible to programmatically customize the
packet processing pipelines in the data plane---enabling execution of a 
subset of dataflow operators at line-rate in the data plane itself. However, 
executing dataflow operators in the data plane requires
maintaining additional state. Thus, \system performs 
{\it query partitioning}, \ie~it executes a portion of a given query over data plane
targets (conventional, OpenFlow, or PISA targets) and the remainder over
streaming targets (Spark, OpenSOC), aiming at striking a balance between 
the workload that the streaming target has to process and the amount of state that
the data plane has to maintained.

Second, we notice that the network traffic that is ``relevant" or  ``interesting" 
for any particular telemetry analysis task usually consists of only a
small fraction of the overall traffic. Thus, network telemetry systems should
support flexible data collection mechanisms that are informed by real-time analysis
results and provide an efficient method for ``zooming-in" during the next time interval
on the portion of traffic that the analysis stage has been deemed ``interesting" in 
the current interval. To enable such dynamic and flexible ``zoom-in" capabilities,
\system performs iterative {\it query refinement}, \ie~it executes queries at 
coarse levels and iteratively executes them over finer levels of granularity for the
portions of traffic that have been identified as interesting. By doing so, it is able 
to winnow out the (bulk of) uninteresting traffic in each iteration, trying to strike
a balance between the overall compute resources required to execute the query and
the total amount of time it takes to identify the traffic that satisfies the query.

To decide how to best partition and refine each query, \system periodically 
collects representative training data from the network and {\em learns} the 
partitioning and refinement plans for each query by trying to “right-size" 
the portions of a query that ought to be executed in the data plane and 
stream processor, respectively, while obeying system-specific limits on
compute resources and operator-specified constraints on detection delay.

\begin{figure}[t!] 
\centering \includegraphics[trim=0 180 380 0,clip,width=\linewidth] {drawings/new-arch.pdf} \caption{\system has three major components:
(1)~Query Interface,  (2)~Runtime System, and (3)~Target-specific Drivers. 
\label{fig-arch}}
\end{figure}

%Figure~\ref{fig-arch} shows \system's architecture. Network operators express 
%queries over packet tuples using \system's API. \system's runtime determines the
%right refinement and partitioning plans for each query. It then sends the partitioned
%queries to the respective target-specific drivers where the corresponding dataflow
%operators get compiled to target-specific configurations. For example, the driver for
%PISA targets compiles partitioned dataflow queries to a P4 program~\cite{P4}. In
%the data plane, incoming packet goes through the packet processing pipeline
%and a subset of them are mirrored and sent to the streaming target. 
%A packet parser captures these packets from the data plane and parses them
%as collection of arbitrary fields amenable to the streaming target. 

Our main contributions can be summarized as follows:
\begin{itemize}
%\itemsep=pt
\vspace{-0.3cm}
\item Design of a unified query interface that lets network operators 
express monitoring queries using a familiar programming paradigm that couples
the collection and analysis stages of (packet-level) network telemetry.
(Section~\ref{sec:applications}). 
\item Design and implementation of a runtime system that uses (1)~query
refinement and (2)~query partitioning to scale the execution of network telemetry
queries (Section~\ref{sec:scale}). 
\item Design \& implementation of a learning module that selects the best 
partitioning and refinement plan for executing each query (Section~\ref{sec:learning}).
\item  Design \& implementation of modular data plane drivers that can execute
a subset of dataflow operators in the data plane (Section~\ref{sec:drivers}).
\item Evaluation that uses realistic monitoring queries, real-world traffic traces, 
and a \system prototype to quantify performance gains (Section~\ref{sec:eval}). 
%\item Publically accessible, open-source implementation with instructions
%for network operators to express and test network monitoring queries in a
%testbed environment~\cite{sonata-github}
\end{itemize}
\noindent


==> learning.tex <==
\section{Selecting Query Execution Plans}
\label{sec:learning}
%In this section, we first make the case for why learning enhances
%\system's ability to scale.  Next, we formalize the learning problem we seek to
%solve and then present our learning algorithm that identifies the best execution
%plan for each input query.

Partitioning, refinement, and sketching enable scalable execution of \system
queries.  For each of these scalability dimensions, \system must choose specific
partitions, refinement plans, and sketch sizes for each query.  For a single
query, there exists many possible combinations of our scalability dimensions and
selecting a poor combination might actually worsen system performance.  We call
the specific set of choices for each of the scalability dimensions a {\em query
plan}. Each plan will require different amounts of resources from the streaming
and the data plane targets and each plan will incur a different detection delay
based on the number of refinement levels. In this section, we describe how the
runtime selects the best plan among all the possible candidates for each
query.

%\begin{figure}[t!] \centering \includegraphics[trim=0 430 550 0,clip,
%width=.9\linewidth] {drawings/system_limits.pdf} \caption{System constraints. 
%\label{fig-limits}}
%\end{figure}

\subsection{The Case for Learning}
\label{ssec:strawman}
Let us first consider fixing each of the scalability dimensions with a uniform 
{\em query plan} applied to all queries.  Such a plan would use a fixed sequence
of refinement levels (pre-determined based on the hierarchy of the fields
selected in the query~\ie, {\tt dns.qname}, {\tt dstIP} etc.), a fixed
partitioning plan, and sketches with fixed sizes based on the counted fields.
However, choosing such an approach would negate the potential benefits of
iterative refinement. The point of iterative refinement is to winnow out 
uninteresting traffic~\ie, that which does not satisfy a query at coarser
refinement levels.  This approach reduces the state required in the data plane
and reduces the number of tuples processed at the stream processor. However, the
efficacy of refinement is not uniform over {\em all possible} refinement levels.
Different refinement levels will winnow out traffic at varying degrees of
effectiveness depending on the fields used as keys for {\tt reduce} and {\tt
distinct} operations, the threshold values for {\tt filter} operations, and the
workload-specific subset of traffic over which the query is applied. If a given
query plan iterates over refinement levels that do not effectively filter out
the uninteresting traffic, then both detection delay and state in the data plane
are increased. Sketch-based data structure performance would also decrease
because their guarantees on accuracy rely on an estimate of the true count of
elements to be stored therein. Therefore in order to determine which query plan
strikes the right balance of costs given the system and query-specific
constraints, we need training data collected from the network. The runtime uses
this training data to learn the optimal query plan that minimizes costs and
satisfies the constraints.

%Although \system employs techniques like refinement and partitioning in order to
%achieve scalability, the performance benefit of these techniques is still
%workload dependent.  For instance, choosing a given refinement level {\tt
%dstIP/}$x$ will yield the most scalability benefits if $x$ correctly sizes the
%aggregate count buckets.  Given the fact that the IPs \system will observe is
%highly workload dependent, we need to train \system to learn the optimal query
%plan for the set of queries it has been issued {\em with respect to the expected
%workload}.

\begin{table}[t]
\begin{footnotesize}
\begin{tabular} {| m{.1 in} m{2.7in} |}
\hline
% & {\bf Queries} \\
$Q$ & Set of input queries expressed using \system's API\\
$W$ & Interval for windowed operations for each query\\
$D_{max}$ & Max. detection delay specified for each query\\
% & {\bf Training Data} \\
$T$ &  Training data collected for $M$ window intervals\\ 
% & {\bf System Constraints} \\
$B_{max}$ & Max. state (bits) data plane can support\\
$N_{max}$ & Max. tuples that the streaming target can process in $W$ seconds\\
\hline
\end{tabular}
\end{footnotesize}
\caption{Input for Learning Problem}
\label{tab:input} 
\end{table}

\subsection{Selecting Query-Specific Plans}
\label{ssec:problem-form}

\smartparagraph{Goal.}
The runtime system's goal is to determine the best query plan for each input
query. Table~\ref{tab:input} summarizes the information available to the runtime
to select the query plan that requires minimal resources and satisfies system
constraints. Let us first introduce the notion of a refinement key ($K$).  A
refinement key consists of a specific header field and a set of levels $\{k_1
\dots k_n\}$ where $k_1$ is the coarsest level and $k_n$ is the finest; thus,
$k_1 > k_n$ implies that $k_n$ is ``finer'' than $k_1$. The meaning of the $n$th
refinement level is specific to each key \eg, in the case of an IPv4 address,
the $k_1$ refinement level would be a {\tt /1} mask applied to the address. In
the case of a domain name, the $k_1$ refinement level would be the root domain (
{\tt "."}) and the $k_n$th refinement level would be a fully qualified domain
name. Refinement plans start at the coarsest refinement level and successively
apply finer choices of refinement, and end at some finest level.  If we think of
all the specific combinations of refinement levels and partitioning plans as
vertices in a graph, then all possible paths from the coarsest to the finest
refinement level become the {\em candidate query plans}. Better yet, the optimal
query plan becomes the shortest-path with minimum cost in the graph of candidate
query plans. We, therefore, choose to frame our learning problem in
graph-theoretic terms.  

%\smartparagraph{Definitions.} We are given training data $T$ that is representative
%of the underlying traffic workload and a set of queries $Q$ expressed using
%\system's API.  We are also given system constraints (see Figure~\ref
%{fig-limits})~\ie, maximum number of packet tuples that the streaming
%target can process ($N_{max}$) and the maximum number of bits that the target
%data plane has at its disposal for supporting stateful dataflow operations ($B_
%{max}$ bits). Lastly, for each query, we are also given a maximum detection
%delay ($D_{max}$). 

\smartparagraph{Enumerating Candidate Query Plans.}
%To formulate our learning problem, we refer to any sequence of successive
%refinement levels (from coarsest to finest) and partitioning choices as a {\em
%candidate query plan}.  
Candidate query plans are paths embedded in a {\em query plan graph} ($g$). 
Before we can describe the structure of this graph, let us first enumerate
other sets from which we will construct the vertices of this graph. For each
query $q \in Q$, let $K_1,K_2,\cdots K_m$ represent the ($m$) candidate
refinement keys in $q$.  The set of all possible refinement levels then
is denoted by $\mathcal{R}=K_1 \times K_2 \times \cdots K_m = \{(k^1, k^2, \cdots
k^m) \mid k^1 \in K_1, k^2 \in K_2, \cdots k^m \in K_m \}$. Therefore, when a
refinement level ($r \in \mathcal{R}$) is an $m$-tuple, $r_j$ is ``finer'' than
$r_i$ if and only if $k_i > k_j$ for one of the constituent keys in the tuple.
The set of all possible consecutive window intervals then is defined as
$\mathcal{I} = \{1, 2, \cdots |\mathcal{R}|\}$.
%\footnote{To simplify notation, we avoid using
%subscripts to indicate the dependency of the sets $R$, $L$, and $\mathcal{P}$ on
%$q \in Q$. The set, $\mathcal{P}$, is also dependent on the data plane target.}
The maximum number of window intervals is initially set equal to the number of
possible refinement levels. However, any query plans that iterate over more
intervals than $D_{max}/W$ (\ie, the maximum detection delay that can be
tolerated for the query) will later be screened out for exceeding a system
constraint. Finally, $\mathcal{P}$ is the set of partition choices, which are
the different ways that $q$ can be partitioned to the data plane. 

All possible combinations of refinement levels and partitioning plans that are 
executed in consecutive window intervals can then be expressed as three-tuples
of the form $\{(r,p,i) \mid r \in \mathcal{R}, p \in \mathcal{P}, i \in \mathcal
{I}\}$ and constitute the vertices in the query plan graph. The query plan graph
is constrained by two requirements: (1)~edges are permitted only from vertices
with coarser refinement levels to finer ones, and (2)~from vertices in the $i^
{th}$ window interval to vertices in the $(i+1)^{th}$ window interval. 
Therefore, two vertices are connected by an edge in this graph if and only if
they are direct neighbors in a candidate query plan. After adding all the edges
that satisfy the above requirements, we discard all the disconnected vertices to
obtain the final query plan graph $g = (V_g , E_g)$ for query $q$. We also
define a globally ``coarsest'' vertex ({\tt Src}) and a globally ``finest''
vertex ({\tt Tgt}) as the source and sink for every candidate refinement plan as
vertices in $V_g$.

\begin{figure}[t!] \centering \includegraphics[trim=0 200 610 0,clip,
height=.8\linewidth, width = .9\linewidth] {drawings/shortest_path.pdf} \caption{
Query plan graph for Query~\ref{asymm-query}. Here refinement levels are 
$\mathcal{R}=\{${\tt dstIP/8}, {\tt dstIP/32}$\}$, partitioning plans are $P=\{1,2\}$, and 
iteration rounds are $\mathcal{I}=\{1,2\}$. 
\label{fig-hgraph}}
\end{figure}

To illustrate, Figure~\ref{fig-hgraph} shows the query plan graph for 
Query~\ref{asymm-query} with the above-defined sets $\mathcal{R}$, $\mathcal{L}$
and $\mathcal{P}$. For ease of illustration, let us consider that we only have
two choices for refinement levels, \ie~$\mathcal{R} =$ \{{\tt dstIP/8}, {\tt
dstIP/32}\}, $\mathcal{I} = \{1, 2\}$, and only two partitioning choices,
\ie~either execute all dataflow operators for the query over data plane target,
or all over the streaming target. Note that in this example, there is no edge
between nodes {\tt  (dstIP/32},{\tt 1},{\tt 1}) to {\tt (dstIP/8},{\tt 1},{\tt
2}) because we only allow zoom-in from a coarser to a finer refinement level in
successive iterations. Not shown are the disconnected nodes we discarded ({\tt
dstIP/8},{\tt 1},{\tt 2}) or ({\tt dstIP/8},{\tt 2}, {\tt 2}) from the final
query plan graph shown in Figure~\ref {fig-hgraph}. Every path in this graph
from {\tt Src} to {\tt Tgt} represents a candidate query plan, therefore, we
have six candidate query plans in this example. 

%\begin{algorithm}[t]
%\begin{algorithmic}[1]
%\Function{Gen-Hypothesis-Graphs}{${\boldsymbol Q}, {\boldsymbol T}$}
%%\State $R = \Call{Get-Refinement-Levels}{Q}$
%%\State $P = \Call{Get-Partitioning-Plans}{Q}$
%%\State $L = \Call{Get-Iteration-Levels}{R}$
%\State $V = \Call{Get-Vertices}{}$
%\For {$m = 1$ \textbf{to} $M$}
%\State $E_m = []$
%\For{$(i,j) \in V.V$}
%\State $ (r_i,p_i,l_i) = V_i, (r_j,p_j,l_j) = V_j$
%\If{$l_{j} = l_{i}+1$ \& $r_{i} < r_{j}$}
%  \State $b,n = \Call{Get-Cost}{Q, T_m, r_i,r_j, p_j}$
%  \State $d$ = $1/|L|$
%\State $\Call{Add-Edge}{E_m, V_i \rightarrow V_j, (b,n,d)}$
%\EndIf
%\EndFor
%\State $G_m = (V,E_m)$
%\EndFor
%\State \Return $G$
%\EndFunction
%\end{algorithmic}
%\caption{\label{alg:generate_graph} Generating Query Plan Graphs}
%\end{algorithm}

\smartparagraph{Weighted Query Plan Graph.} 
For a given query and training data, the weight for each edge in the resulting 
query plan graph $g =(V_g ,E_g)$ is determined by the two primary cost metrics 
described in Section~\ref{sec:scale}. In particular,
the number of packet tuples $n$ and bits $b$ associated with an edge
between nodes ($i,j$) is determined by executing the query for refinement
level $r_{j}$ and partitioning choice $p_{j}$ over the training data.  These
costs are calculated after filtering out the traffic that does
not satisfy the query at refinement level $r_{i}$.
Note that these costs only depend on how well the traffic
not-satisfying the given query was winnowed out at refinement level ($r_{i}$)
before getting executed at refinement level ($r_{j}$) with a partitioning plan
$p_{j}$. 
%In particular, these costs do not depend on the iteration rounds, $l_i,
%l_j$, or on how the query was executed before ($p_i$). As a result, all the
%edges with similar $r_i, r_j, p_j$ values will have the same costs. 
%As for the
%third cost metric (\ie~detection delay ($d$)), it is equal to $W$, a given
%window of time, and 
Both these cost metrics are normalized with respect to the
given bounds $N_{max}$, and $B_{max}$.

Finally, we combine these different cost metrics linearly to define the
normalized weight $w$ for every edge in the query plan graph~\ie, $w =\alpha n+
(1-\alpha)b$. Here, $\alpha \in [0,1]$ is a tunable parameter that assigns
relative importance to the two cost metrics. For example, setting $\alpha = 0$
implies that the learning problem is indifferent to the number of packets
processed by the streaming target but is maximally concerned with the number of
bits required to execute stateful dataflow operations in the data plane and
vice versa.
%Similarly, setting $\beta=0$ implies that the learning problem is insensitive 
%to the number of iterations and therefore indifferent to detection delay.

These weight computations result in a {\em weighted} query plan graph $g_w$
where the cost of each path (i.e., candidate query plan) between
the {\tt Src} node at the coarsest level and the {\tt Tgt} node at the finest
refinement level is defined as the sum of the (normalized) weights of the edges
on that path, \ie~$\sum_{e} \alpha n_e+(1-\alpha)b_e$ for all edges $e$ in
the candidate query plan.


%while the core query plan graph ($g$) for query $q$ remains constant for each of
%the $M$ values, but the weighted graphs ($g_w$) will vary across the different
%training data sets.


%\subsection{Learning Query Plans}
%\label{ssec:single-learn}
\subsection{Learning Algorithm}
We compute the weight of each edge for every window interval. 
As the duration of training data is $M$ window intervals, this for each $m \in 
[1,M]$,  we use training data $T_m$ to generate a weighted query plan graph for
query $q$. This way, we obtain a total of $M$ different weighted query plan
graphs. Note that for different time intervals, $m$, only the weight of
individual edges changes. For each window interval $m$, we can apply the {\em
Dijkstra} algorithm over the weighted graph to find the plan with minimum cost.
However, for each time intervals, the edges in the graph will have different
weights. Therefore, different time intervals are likely to have different
minimum-cost query plans. The goal of the learning algorithm is to find the
query plan that best fits all of the training data over all time intervals. 
Therefore, we select the candidate query plan ($p$) that minimizes the root-mean
square error where $p_i$ below represents the minimum-cost query plan for
interval $i$.$$RMSE(p)=\sqrt{\frac{1}{n}\sum_{i=1}^{m}{(cost(p)-cost(p_{i})})^2}$$

To avoid overfitting the data, we rely here on a common practice when solving 
(supervised) machine learning problems; that is, we ``hold out" parts of the
available training data as test data and apply basic {\em K-fold
cross-validation} to learn the best query plan. 

\smartparagraph{Tuning $\alpha$.}
As mentioned earlier, the tunable parameter $\alpha$ assigns relative 
importance to the normalized $N$ and $B$ costs. As we increase $\alpha$,
we trade off higher cost $N$ for lower cost $B$. For the given system
constraints, \ie~$N_{max}$ and $B_{max}$, each value of $\alpha$ can result in
four possible states depending on whether cost $N$ is greater/less than $N_
{max}$ and cost $B$ is greater/less than $B_{max}$. To tune $\alpha$, 
we start with $\alpha = 0.5$ (equal weight to normalized $N$ and $B$ costs) 
and perform a binary search with the goal of finding an $\alpha$-value where the 
weighted cost of the query plan across all $M$ intervals
is minimum while ensuring that the constraints $N \le N_{max}$ and $B \le B_{max}$ 
are satisfied for each candidate $\alpha$. Note that no feasible solution exists if any
$N > N_{max}$ and $B > B_{max}$.

We use this approach as an illustration, but other more complex (supervised) machine
learning algorithms can readily be substituted to learn the best query plan and tune 
$\alpha$, using the training data and system constraints. 

%For each query plan graph, we first determine the best query plan by applying a 
%{\em uniform cost search algorithm} that determines the minimum cost path. We
%then set $K=M/10$ and apply K-fold cross-validation; that is, for each fold (or
%partition of the training data) $F_k (k \in [1,\cdots,K])$, we first use $K-1$
%of the folds as training data and identify the query plan that is best for a
%majority of these $K-1$ folds---we call this $F_k$'s training query plan. Then we compute 
%the root mean square error that results from applying $F_k$'s training query plan over 
%the validation set (i.e., the fold we held out)---we call this $F_k$'s validation error 
%denoted by $Err_{F_k}$. Finally, we select as best query plan the training query plan 
%that has minimum error across all $K$ folds.  Although network traffic (\ie,
%both the traning and validation sets) can vary with diurnal and unpredictable
%fluctuations, we can avoid learning these biases by periodically relearning the
%best query plan.


%\smartparagraph{Queries with multiple refinement keys.} 
%Our example in Figure~\ref{fig-hgraph} considers only a single refinement key
%~\ie, {\tt dstIP}. However, in practice, there can be more that one candidate
%refinement key for a query~\eg, {\tt dstIP}, {\tt srcIP} for Query~\ref
%{asymm-query}. Supporting multiple refinement keys requires updating the set of
%candidate refinement levels $R$ to include combinations of refinement levels for
%each refinement key instead of a single value. For example, if the refinement
%levels for IP addresses are configured to iterate at levels \{{/8, /32}\}, and
%if we are considering both {\tt dstIP} and {\tt srcIP} for iterative refinement
%for Query~\ref{asymm-query}, then the runtime will enumerate the set of
%refinement levels as $R=$ \{({\tt dstIP/8}, {\tt srcIP/8}), ({\tt dstIP/8}, 
%{\tt srcIP/32}), ({\tt dstIP/32}, {\tt sIP/8}), ({\tt dstIP/32}, {\tt
%sIP/32})\}.

%\smartparagraph{Queries with {\tt Join} operations.}
%As we discussed in Section~\ref{sec:scale}, a {\tt join} operation is executed
%over two consecutive window intervals in the data plane, where the 
%output of the first query is served as a filter to the input of the second
%one at the end of each window interval. Thus for queries with {\tt
%join} operators, each iteration in the query plan graph increments delay by two
%window intervals. 
%%This also implies that the query partitioning decisions are
%%independent for the two joined queries, which results in additional partitioning 
%%plans ($\mathcal{P}$) for these queries.



\smartparagraph{Learning for Multiple Queries.} 
Multiple queries compete for limited resources~\ie, the amount of state in the
data plane and processing power at the streaming streaming targets. The
problem of finding the right query plans for all queries that require minimum
resources and also satisfy the system constraints, can be mapped to the {\em bin
packing problem}~\cite{bin-pack}, and is thus an NP-hard problem. We designed a 
simple greedy algorithm for multiple queries that tunes a single value of
$\alpha$ for all queries together, which is a simple extension
of our algorithm for the single query case. It performs a binary search
exploring the value of
$\alpha$ that minimizes the total weighted cost and applies the constraints over the
total number of bits and tuples for all the queries. Clearly, this algorithm
will not find the optimal solution where different values of $\alpha$ for
different queries might minimize the total weighted cost. 

%In our current solution, we configure independent packet processing pipelines 
%in the data plane---maintaining separate hash tables for each query. However, it 
%is possible to share some match/action tables and registers across different operators of the input
%queries---making better use of available resources. The problem of designing
%such packet processing pipelines and learning  the right execution plans for
%such a setup is exciting, but is beyond the scope of this work. We leave this as
%problem for future work. 


==> overview.tex <==
\section{\system's Design}
\label{overview}
%In this section, we will provide an overview of \system. Figure~\ref{fig-arch}
%shows its three major components: (1)~a unified Application Interface that allows network operators
%to express their monitoring queries without worrying about {\em where} and {\em how} their
%queries get executed, (2)~a Runtime system that determines {\em where} each user query
%gets executed, and (3)~Dataplane \& Streaming Drivers, that determine {\em how} partitioned
%sub-queries get executed over a range of data plane and streaming targets.

Network Telemetry describes how information 
from various data sources can be collected using a set of automated communication 
processes and transmitted to one or more receiving equipment for analysis tasks. 
Analysis tasks may include event correlation, anomaly detection, performance monitoring, 
metric calculation, trend analysis, and other related processes~\cite{telemetry2016big}.
Detecting events of interests in real-time typically requires {\em packet-level granularity},
\ie~examining network behavior at the granularity of individual packets. 

\begin{figure}[t!] \centering \includegraphics[trim=0 200 300 0,clip,
width=\linewidth] {drawings/new-arch.pdf} \caption{Sonata's
architecture for detecting network events in reactive manner.\label{fig-arch}}
\end{figure}


\subsection{Unified Query Interface}
\label{ssec:abstraction}
Our goal is to provide network operators with an interface that makes 
it easier for them express queries----analysing traffic at packet-level 
granularity w/o worrying about {\em where} and {\em how} they queries 
get executed. 

Network operators have traditionally applied the logical division of network 
telemetry into a {\em collection} stage and an {\em analysis} stage.  Most
tools either perform collection or analysis tasks---leaving it to the network
operators to manually stitch these tools together for network telemetry. 

For the collection stage, network operators must grapple with how to
gather information from a distributed set of collectors to some centralized location. 
To support the analysis at packet-level granularity, solutions that collect
and mirror raw packets from the wire for analysis are deployed. However,
these solutions don't scale as the traffic volume increases in the data plane.

Typically, operators employ tools that transform the
data at the distributed collectors to some aggregated statistical values (e.g.,
per-link counters) and then use fixed protocols (\eg~SNMP) for central
collection. Alternatively, tools can locally reduce the data to a randomly
sampled subset of the original data and again use fixed protocols (\eg~NetFlow,
IPFIX, etc.) for central collection. While these approaches succeed in
decreasing the volume of the data that is transferred for
analysis, the loss of information due to such data reductions is, in general, too
severe and prevents any meaningful real-time decision-making based on the
collected data.~\footnote{Note that the definition of {\em real-time} is
different for different networks. In wide-area settings where high latency
values dominate, it is reasonable to consider detecting events within a few
seconds as real-time. This is different for data center networks where detection
within a few milliseconds is considered as real-time.} 

For analysis, operators have typically relied on protocol-specific tools, or more
recently they embraced the {\em Dataflow} programming model that applies
sequence of transformation over set of tuples~\cite{opensoc, }. However, the 
analysis stage is tightly coupled with the collection stage. Network operators have 
to express different queries for different collection tools.
For example, the query to analyse raw packet captures can't be applied over the
SNMP data. Any changes to the collection platform requires network operators
to change their existing analysis queries---making the system brittle. 

\smartparagraph{ Packets As Tuples.}
In {dataflow} programming model, tuples can represent arbitrary unstructured 
data. Conveniently, packets can be also represented as tuples. Our programming
abstraction lets network operators express their queries over packet tuples using 
dataflow programming model itself.
It hides the details of how \system scales the exeution of these queries. It also
hides the details of the underlying targets that execute their queries. 

Each packet tuple is a collection of arbitrary field values including but not limited 
to header fields like {\tt srcIP}, {\tt srcMac}, {\tt srcPort}, {\tt dstIP}, {\tt dstMac}, {\tt dstPort},
{\tt payload}, etc., and payload fields like ({\tt dns.aIP}, {\tt dns.domain},
etc.). In order to support a richer set of queries, a packet's tuple entries may also
include metadata such as: (1)~{\tt size}, which specifies the packet's size in
bytes; (2)~{\tt locationID}, which specifies the packet's unique location in the
network (\eg~unique port number~\cite{}); (3)~{\tt queueSize}, which specifies
the length of the queue at a particular location when the packet traversed that
location. In Section~\ref{sec:applications}, we describe how network operators 
can use this programming abstraction to express wide-range of network monitoring
queries. 

%Note that even though the programming abstraction supports arbitrary fields in the
%packet tuple, the ability to execute queries over these tuples depends on
%the underlying hardware. For example, not all data plane devices can extract
%queue size information.  Section~\ref{} provides more details on how \system
%determines whether it can execute a given input query or not. 

\subsection{Scalable Execution}
The runtime system receives monitoring queries expressed by the network
operators. Its primary goal is to ensure that \system is able to scale the execution 
of wide-range of network monitoring tasks expressed as dataflow queries applied 
over packet tuples.



\smartparagraph{Challenge.}
Typically, dataflow queries are executed over general-purpose compute nodes.
Executing \system queries over general-purpose compute nodes requires
mirroring, capturing, and parsing (collection stage) all the data packets in the network 
before applying the dataflow queries (analysis stage). While ``scaling out” 
the collection stage is possible~\footnote{There are commercial products
capable of performing lossless packet capture at link speeds of 100 Gbps and
beyond~\cite{niksun}.}, ``scaling out” the analysis stage has its limits. Even
though modern stream processing platforms are designed to scale linearly, the
cost and complexity of processing hundreds of millions of packet tuples for just
one query is simply too high to work in practice~\cite{osoc-scale}. 

\smartparagraph{Query Partitioning.}
Execution of \system queries can be scaled if we can offload some of the
dataflow operations to the data plane. Executing datflow queries in the dataplane
requires: (1)~programmable parsing, \ie~ability to parse/deparse arbitrary 
query-specific header fields, (2)~state management primitives, \ie~ability
to maintain arbitrary query-specific state in the data plane, (3)~flexible match/action
table pipelines, \ie~ability to combine different tables (executing dataflow operators)
in arbitrary query-specifc order. 

Most data plane targets do not support any of these features and only support
limited fixed transformations in the data plane. SDN-based dataplane targets
can support flexible match/action table pipelines, and can thus support few
dataflow operators like {\tt filter, sample} in the data plane. However,  recently 
proposed {\em Protocol Independent Switch Architecture (PISA)} switches (see Figure~\ref
{fig:pisa}) provide many features that permit the implementation of customized
packet processing and state management logic in the data plane~\cite{rmt,
p4-xilinx, barefoot-blog, P4, p4-netronome}. By supporting the execution of a 
subset of {\em dataflow} operations in the data plane itself, PISA features permit the 
critical integration of the collection and analysis stages. In section~\ref{ssec:qpart},
we describe the challenges and limitations of executing  dataflow queries
in data plane. 

\smartparagraph{Iterative Refinement.}
Many network monitoring tasks involve identifying anomalies in network traffic. 
In many cases, the traffic of interest is only a small fraction of the total traffic.  
By continuously running network monitoring queries over all the incoming 
packets, we end up wasting resources on traffic that is mostly uninteresting 
for the given query. We observed that it is possible to leverage the hierarchical 
structure of some of the fields in the packet tuple by first executing the query 
at a coarser levels of refinement and then iteratively zooming-in at finer 
levels---winnowing out the traffic that does not satisfies the query at the coarser 
levels. In section~\ref{ssec:ir}, we describe the challenges and limitations of
iterative refinement.

\smartparagraph{Learning Query Plans.}
There can be multiple plans for executing \system queries, \ie~different
sequence of refinement levels and different partitioning plan for each level. Each plan
will have a cost, and these cost will vary for different queries operating under
different workloads. Thus, it is required to determine the execution plan with minimal cost 
for each query given traffic workload. Section~\ref{sec:learning} describes the learning
problem and solution that takes system constraints and representative training 
data as input to learn the best plan for each query.  


%\smartparagraph{Runtime System.}
The runtime system interacts with the underlying data plane and streaming drivers
to enumerate possible execution plans for each query.  It then uses training
data and a cost model (from target-specific drivers) to evaluate the cost of
different plans, and finally applies a learning algorithm to search the 
plan with minimum cost. Once it learns the execution plan for a query, it sends
refined and partitioned sub-queries, from the input queries, to the
corresponding drivers. 
The runtime system is also responsible for handling the output of each query at
the end of window intervals---(1)~publishing results for network operators,
and/or (2)~updating queries to enable iterative refinement. 


%Few existing solutions, like OpenSketch~\cite{opensketch} and Univmon~\cite{univmon},
%apply similar transformations to the packet stream in the data plane. However, they
%require the network operators to explicitly program the 
%However, unlike 
%\system, they do not support the packet-as-tuple abstraction---requiring network operators to
%express limited set of target-specific queries. 
%
%In past, few solutions like , explored the idea of iterative refinement. However, 
%most of these solutions were very specific to a limited set of monitoring queries.



\subsection{Support Target Diversity}
Drivers receive partitioned sub-queries and are primarily responsible for 
determining {\em how} to execute (compile/update) these queries. They are 
also responsible for exposing target-specific information that is required by the 
runtime to learn the optimal query plan. Table~\ref{tab:driver-api} shows the
driver API exposed to the runtime system. 

\smartparagraph{Dataplane \& Streaming Targets.}
Targets are the components that actually execute the partitioned sub-queries.
Dataplane targets can range from devices based on traditional fixed-function
chipsets, to more flexible Software Defined Networking (SDN) switches,
\eg~OpenFlow, to ones that use reconfgurable chipsets, \eg~PISA targets.
Streaming targets can range from ones that adopt the bulk-synchronous parallel 
(BSP) model for data processing, \eg~Apache Spark, to the ones that adopt the
record-at-a-time streaming model,~\eg~Apache Flink.  Whatever the target, as
long as it implements the API in table~\ref{tab:driver-api}, \system can
incorporate it.



\smartparagraph{Packet Parser.}
The data plane driver not only configures the underlying dataplane devices, but it
also configures a {\em packet parser}. This parser is responsible for decoding
the incoming packet stream of raw packets, sometimes with embedded custom
fields, and emitting them as a tuple of strings to the stream processor. Notice
that configuring this packet parser is related to the question of {\em how} to
execute a given query and is thus configured by the data plane driver and not the
runtime system. 










==> scalability.tex <==
\section{Query Compilation with PISA Targets}
\label{sec:scale}
In this section, we describe how modern Protocol-Independent Switch
Architecture (PISA) switches can execute dataflow operations in the
data plane.  Next, we show how to partition a query to perform some
operators in the switch and the rest at the stream processor.  Then,
we present techniques for reducing overhead, by allowing bounded delay
or error in answering queries.

%We first explore the different choices runtime has 
%for executing operators' queries. We then describe how it compares these
%choices and selects a plan striking balance between different cost metrics. 
%
%%focus in this section on {\em Query Partitioning}
%%and {\em Iterative Refinement} as the two key ideas that ensure the desired 
%%scalability property of \system.

 
% \begin{table}
% \noindent
% \begin{minipage}{\columnwidth}
% \lstset{belowskip=0pt}
% \begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
% caption=P4 code that executes {\tt filter} operation over PISA targets., 
% captionpos=b, label=stateless-dp-operators, captionpos=b,
% basicstyle=\footnotesize, 
% numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
% table filter {
%  reads {srcPort: exact;}
%  actions{pass; drop;}
%  }
% \end{lstlisting} 
% \end{minipage}\hfill
% \begin{minipage}{\columnwidth}
% \lstset{belowskip=0pt}
% \begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
% caption= P4 code that executes {\tt distinct} operation over PISA targets., 
% captionpos=b, label=stateful-dp-operators, captionpos=b,
% basicstyle=\footnotesize, 
% numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
% register D{width:1; instance_count: B;}
% action do_read() {
%  modify_field(idx, 0, H(dstIP, srcIP), B);
%  register_read(val, D, idx);}
% action do_update() {
%  bit_or(val, val, 1);
%  register_write(D, idx, val);}
% table read {actions {do_read;}}
% table update{actions {do_update;}}
% control distinct {
%  apply(read);
%  if (val == 0) {
%   apply(update);} 
% \end{lstlisting}  
%  \end{minipage}\hfill
% \end{table}

\subsection{PISA: Enabling Dataflow Operations}
\label{ssec:pisa}
Traditional network devices do not support custom packet processing or
state management in the data plane.  In contrast, recently introduced
PISA targets~\cite{rmt,p4-xilinx,barefoot-blog,P4,p4-netronome}
provide many features that can support dataflow operators directly
in the data plane.

\smartparagraph{Programmable parsing.}  PISA targets allow for the
specification of new header formats for parsing
%JEN: omitting deparsing, as it is not (yet) defined
%and deparsing
packets.  Programmable parsing enables both the extraction of desired
header fields for answering arbitrary queries and the definition of
application-specific header formats for sending streams of tuples to a
stream processor.

\smartparagraph{State in packets and registers.} Queries may require
per-packet state (\eg, {\tt qSize}) or calculations for other dataflow
operations. Such fields are easily implemented in user-defined
metadata. Additionally, queries often require accumulating statistics
across a sequence of packets (\eg, a sum in a {\tt reduce}
operation). PISA targets have rule tables that maintain byte and
packet counters, as well as more general registers that can perform
simple computations to update state.

\smartparagraph{User-defined hashing.} Operators like {\tt reduce} and {\tt distinct} require 
maintaining state in the data plane that depends on combinations of {\em
query-specific} reduction keys. Support for hash calculations over query-defined
field combinations allow these operators to maintain the required state in the
data plane.

\smartparagraph{Flexible match/action table pipelines.} Flexible match
action tables in the reconfigurable data plane ensure that novel
combinations of dataflow operators can be applied to the right subsets
of matched packets.

\subsection{Reduce Processing: Partitioning}
\label{ssec:choices}
To reduce overhead, \system performs some portions of a query directly
in the data plane, and relies on the stream processor to perform the 
remaining operations. 
%JEN: unnecessarily leading...
% \system's runtime system relies on a dataplane
%driver to determine what subset of dataflow operators a particular data plane
%target can support and at what cost.  With this information,
For a PISA data plane target, \system can implement the following
operators directly in the data plane.

\smartparagraph{{Map}, {filter}, and {sample} operations.}  Filter
operations, like line 2 of Query~\ref{asymm-query}, match on fields in
the packet's header. Naturally, this operation aligns with a
match-action table in the data plane.  For example in Query~\ref
{asymm-query}, line 2 corresponds to a table that matches on the {\tt proto}
field and ignores all non-DNS traffic.  Map and sample
operations can also be executed using similar match-action tables each
applying different actions over matched packets. For example, in Query~\ref
{asymm-query}, line 5 corresponds to a table that transforms the {\tt dstIP}, 
{\tt srcIP} pair into a tuple of ({\tt dstIP}, $1$). Finally, {\tt filter}
operations that require evaluating a predicate, as in line 7 of Query~\ref
{asymm-query}, are implemented with two match/action tables: one for each
possible evaluation of the predicate. For all of these operators, the
state required to execute them in the data plane can be quantified
as the size of the match/action tables, \ie, size of fields matched,
and the total number of match entries.  The savings in processing
realized at the stream processor comes at the cost of maintaining this
state in the data plane.


\smartparagraph{Distinct and reduce operations.}
The {\tt distinct} and {\tt reduce} are slightly different from the previous
operations because these operations require maintaining state across sequences
of packets.  In the case of {\tt distinct}, the state maintained is a single bit
indicating whether or not a particular key has already been observed; in the
case of {\tt reduce}, it is the result of applying a function (\eg ~sum) over a
particular (set of) key(s). We use hash tables to maintain state and a metadata
field for storing and updating the values from the hash tables. The state
required for executing these stateful operators in the data plane can be
quantified as the total size of the hash tables used. 

%%JEN: jumps into too much low-level detail, before the high-level idea
%%is sufficiently clear.
%Let us demonstrate how the {\tt distinct} operation, \eg, line
%4 of Query~\ref{asymm-query} is in implemented in a PISA switch.  
%This operator requires storing values in a hash table ({\tt
%register}) and must be split into two stages: {\em read} and {\em update}. In
%the first stage, a {\em read} is performed on each incoming packet. A hash
%function $H$ is applied over the {\tt dstIP}, {\tt srcIP} fields to calculate
%an index $i$ into the hash table. This index is used to lookup the value in
%the hash table and store the value in metadata.  If the packet's {\tt dstIP}, 
%{\tt srcIP} pair has already been observed then the value is one and zero
%otherwise. In the second stage, if the value is zero we {\em update} the value
%and write back to the hash table. More precisely, the {\em update} action first
%applies a  function (in this case, {\tt bit\_or}) over a particular metadata
%field and then writes the updated value to the hash table. The {\tt
%distinct} operator turns out to be a special case of the {\tt reduce} operator
%in which other functions (\eg, {\tt sum}) can be applied instead of {\tt
%bit\_or}. 

%% AG: Not sure of this should go to the implementation section
%As the statefull operators are time-bounded by a window of $W$ seconds.
%Thus, at the end of each window interval, the data plane driver resets the
%hash table values to zero. There are two ways in which state for operations
%like {\tt distinct}, and {\tt reduce} can be reported to the remainder operations
%running over the streaming target. First, {\em batch} compute mode, where we send the 
%updated state at the end of every window interval. This can be achieved by sending 
%special packets, at the end of each window
%interval that reads the state in the hash tables and report the updated
%values to the streaming target. This approach has low compile time complexity
%but higher runtime overhead as it requires sending additional query-specific custom 
%packets at the end of every window interval.  Second, {\em per-packet} compute mode,
%where we append the updated state to the packet itself---reporting a copy of incoming
%packets to the streaming target. Clearly, not all incoming packets need to be reported
%For example, packets for the non-DNS traffic for Query~\ref{asymm-query},
%are not required to be reported to the streaming target. We add an additional 
%query-specific one bit field {\tt report} to each packet. Only the packets for
%which the {\tt report} bit is set to one are cloned and sent to the streaming
%target. The latter approach has higher compile time complexity as it requires redundant
%execution of operators like {\tt reduce}, but has lower runtime overhead. We chose the
%latter approach---trading compile time complexity for runtime overheads. 
%
%% AG: Implementation or this section?
%In {\em per-packet} compute mode, the update state is added to the packet.
%In case of {\tt reduce} operation for Query~\ref{asymm-query} (line 6) the
%updated count is added as a field and reported to the next operators. The
%next operator, \ie~{\tt filter} will ignore the packets below the threshold value.
%However, for all the packets with count greater than the threshold, it will
%report them to the streaming target. Naively partitioning the operators this
%way will result in incorrect output of the query. To avoid reporting incorrect
%query output, we (1)~update the {\tt filter} operation such that it reports the first
%packet that exceeds the threshold with the actual count value and setting
%count to one for all the remainder packets; (2)~redundantly apply {tt reduce}
%and {\tt filter} operations over the streaming target to make sure that final 
%reported output is correct. 


\smartparagraph{Join operations.} Supporting {\tt join} operations in the data plane
is difficult as it entails additional complexity of supporting build and probe
semantics for implementing doubly pipelines {\tt join} operator~\cite
{aqp-survey}. We currently execute {\tt join} operation as {\tt filter} where
the output of the left query from the previous window interval is served as a
filter for the right query. For example, in case of Query~\ref{payload-query},
the output of Query~\ref{asymm-query}, \ie~anomalous {\tt dstIPs} are 
applied as filter operation in line 4 of Query~\ref{payload-query}.

\smartparagraph{Limitations.}
PISA targets cannot support all the dataflow operations for a query 
directly in the data plane. The limited set of parsing actions and computational
capacity limits these targets' ability to support arbitrary dataflow
operations. For example, extracting payload fields and performing arbitrary
regular expression operations over the payload field cannot currently be
supported in PISA targets. Also, only simple computations, like {\tt add} and 
{\tt subtract}, or simple bit manipulations, {\em etc.} can be applied over
tuple fields in the data plane. Thus, operations that require complex
transformations over tuple fields~\eg, a {\tt reduce} operation for entropy 
estimation, requiring logarithmic transformation, cannot be supported in the data plane. 


\subsection{Reduce State: Sketches \& Refinement}
\label{ssec:reduce-state}

Offloading dataflow operations to the switch requires maintaining
additional state in the data plane.  Yet, PISA targets can only store a limited
amount of state. We will now describe
how \system can stay within these space limitations by incurring delay in
answering queries or tolerating bounded error. 


% The biggest difference between executing stateful dataflow operators in the data
% plane is how the memory is provisioned for maintaining state. For streaming targets, the 
% memory required to maintain state can be updated during the execution time itself. 
% However, for data plane targets, it needs to be provisioned before the execution, as 
% shown in line 1 for Query~\ref{stateful-dp-operators}. Provisioning lesser memory
% will result in hash collisions and inaccurate answers. Thus, the size allocated for the 
% registers in the data plane should be more than or equal to the number of unique
% entries expected for each stateful operation to avoid hash
% collisions. 

\textbf{Relaxing latency with iterative refinement:}
Like Query~\ref{asymm-query}, many network monitoring tasks involve identifying
anomalies in network traffic, and in many of these cases, the traffic of interest 
is typically only a small fraction of the total traffic. For example, we 
observed that only 1\% of the total traffic at one of the world's largest 
IXPs constituted DDoS reflection attack traffic. If we continuously run network 
monitoring queries over all the incoming packets, we end up wasting compute
resources and maintaining state for traffic that is of no interest as far as a
given query is concerned.  Instead, we can leverage the hierarchical structure
of some of the fields in the packet tuple, \eg, {\tt srcIP}, {\tt dstIP}, {\tt
dns.qname} etc. and execute queries at coarser levels of refinement for these
fields.  Iterative refinement transforms a single query into a set of queries
that successively zoom-in on traffic of interest.  For example, if we replace
the field {\tt dstIP} with {\tt dstIP/8} for Query~\ref{asymm-query} (see line 3
in Query~\ref{query-transform}), then the number of unique pairs of {\tt dstIP/8}, and {\tt
srcIP} drops significantly. After executing the query at this coarser level, we
can then zoom-in over the interesting traffic that satisfied the query at a
coarser level in the next iteration round (see line 8 in Query~\ref{query-transform}). 
This iterative refinement winnows out the
uninteresting traffic in each round which in turn allows us to dedicate
available compute resources to the portion of traffic that matters for the
query. This process saves state in the data plane but comes at the cost of the
additional detection delay incurred during the iteration.  
\noindent
\begin{table}[t]
\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
caption=Query transformations for iterative refinement,
captionpos=b, label=query-transform, captionpos=b,
basicstyle=\footnotesize, 
numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
Q1_8(t) = pktStream(W)
    .filter(p => p.proto==17)
    .map(dstIP --> dstIP/8)
    .map(p => (p.dstIP, p.srcIP))
    ... 
Q1_32(t) = pktStream(W)
    .filter(p => p.proto==17)
    .filter(p => (p.dstIP/8 in Q1_8(t-W)))
    .map(p => (p.dstIP, p.srcIP))
    ... 
\end{lstlisting} 
\end{minipage}
\end{table}

%\begin{figure}[t] 
%\begin{minipage}{1\linewidth}
%\begin{subfigure}[b]{\columnwidth}
%\includegraphics[trim=0 380 600 0,clip,height=0.3\linewidth]{drawings/single_query_ir.pdf}
%\caption{Iterative refinement in action} 
%\label{fig-single-ir}
%\end{subfigure}
%\begin{subfigure}[b]{\columnwidth}
%\lstset{belowskip=0pt}
%\begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
%captionpos=b, label=query-transform, captionpos=b,
%basicstyle=\footnotesize, 
%numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
%Q1_8(t) = pktStream(W)
%    .filter(p => p.proto==17)
%    .map(dstIP --> dstIP/8)
%    .map(p => (p.dstIP, p.srcIP))
%    ... 
%Q1_32(t) = pktStream(W)
%    .filter(p => p.proto==17)
%    .filter(p => (p.dstIP/8 in Q1_8(t-W)))
%    .map(p => (p.dstIP, p.srcIP))
%    ... 
%\end{lstlisting}  
%
%\label{q32}
%\end{subfigure}
%\end{minipage}
%\caption{Applying the refinement plan [{\tt dstIP/8}, {\tt dIP/32}] for Query~\ref{asymm-query}} 
%\label{fig:ir} 
%\end{figure}


\textbf{Relaxing accuracy with sketches:}
While refinement transforms queries into a set of augmented queries,
sketching transforms a query into a set of data structures in the data
plane. In order to avoid collisions, hash tables are typically both bloated and
sparse.  Instead, we can employ smarter data structures that summarize the
relevant data in bounded memory and with some bounded loss in accuracy. For
example, Bloom filters~\cite{bloom-filters} are compact data structures useful for
set-membership testing.  In the case of the {\tt distinct} operator, we can use
a bloom filter to test whether or not a given key is a member of the ``set of
unique keys''.  For example, in Query~\ref{asymm-query}, at line 4, we create an
array with $m$-rows storing only a single bit in each row.  For a single
input key (\ie, {\tt dstIP} and {\tt srcIP} pair) $k$ hashed indices are
calculated to implement a bloom filter for the ``set of unique keys''.
Similarly when maintaining a count statistic, we can employ a count-min sketch.
This sketch estimates a count statistic by maintaining $k$, $m$-bit wide tables
each indexed using a different hash function.  For example, in Query~\ref
{asymm-query}, we use a separate count-min sketch at line 6 for performing the
reduction operation on the sequence of ({\tt dstIP}, $1$) tuples. By choosing
wise values of $k$ and $m$, we can achieve significant size reduction with
provable accuracy loss~\cite{cms}. The amount of state required for implementing
both of these sketch-based stateful dataflow operations depends on user-defined
error bounds that allow the operator to trade off the amount of state required
with accuracy~\cite{opensketch}.  Additionally, there is no trade-off between
sketching and refinement; we can employ both techniques at the same time to
achieve even better system scalability.
%JEN: the point in the next sentence could be mentioned at the end, as
%each of the two techniques can benefit from the use of the other.







%\begin{figure}[ht] 
%\begin{minipage}{1\linewidth}
%\begin{subfigure}[b]{\columnwidth}
%\includegraphics[trim=0 380 640 0,clip,width=.8\linewidth]{drawings/single_query_ir.pdf}
%\end{subfigure}
%\end{minipage}
%\caption{Applying the refinement plan [{\tt dstIP/8, dIP/32}] for Query~\ref{asymm-query}.
%Query at finer level ({\tt dstIP/32}) is only applied over traffic that satisfies the query at 
%coarser level ({\tt dstIP/8}).} 
%\label{fig:ir} 
%\end{figure}
%
%
%\begin{table}
%\noindent
%\begin{minipage}{\columnwidth}
%\lstset{belowskip=0pt}
%\begin{lstlisting}[language=p4,basicstyle=\footnotesize, 
%caption= Query transformations for iterative refinement, 
%captionpos=b, label=query-transform, captionpos=b,
%basicstyle=\footnotesize, 
%numbers=left,xleftmargin=2em,frame=single,framexleftmargin=2.0em]
%Q1_8(t) = pktStream(W)
%    .filter(p => p.proto==17)
%    .map(dstIP --> dstIP/8)
%    .map(p => (p.dstIP, p.srcIP))
%    ... 
%
%Q1_32(t) = pktStream(W)
%    .filter(p => p.proto==17)
%    .filter(p => (p.dstIP/8 in Q1_8(t-W)))
%    .map(p => (p.dstIP, p.srcIP))
%    ... 
%\end{lstlisting}  
% \end{minipage}\hfill
%\end{table}

%\begin{table}[ht]
%\begin{footnotesize}
%\begin{tabular} {| m{.5 in} m{2.25in} |}
%\hline
%{\bf Constraints} & {\bf Description} \\ \hline
%{$N_{max}$} & Maximum number of packets the streaming target can process in a 
%given window interval.\\
%$B_{max}$ & Maximum number of bits that the data plane can use for executing 
%dataflow operations. \\ 
%$D_{max}$ & Maximum detection delay that the query can tolerate. \\ 
%$P_{max}$ & Maximum error probability for query's output\\ 
%\hline
%\end{tabular}
%\end{footnotesize}
%\caption{System \& Query-Specific Constraints.}
%\label{tab:constraints} 
%\end{table}





%\subsection{Query Partitioning}
%\label{ssec:qpart}
%Query partitioning refers to deciding which subset of a query's different
%dataflow operations to apply over the incoming packet streams in the data plane 
%itself, before sending it to the streaming target. In effect, in query partitioning,
%\system's runtime partitions the input query into two parts and sends the
%first part to the data plane driver and the second part to the streaming driver.
%
%\begin{table}[ht]
%\begin{footnotesize}
%\begin{tabular} {| m{1.0 in} m{1.75in} |}
%\hline
%{\bf Driver API} & {\bf Description} \\ \hline
%{\tt {\bf isSupported}(q,t)} & Returns whether query {\tt q} can be executed
%over the specified target {\tt t}.\\
%{\tt {\bf getCost}(q,d,t)} & Returns normalized cost of executing query
%{\tt q} over the specified target {\tt t}, given training data {\tt d}. \\ 
%{\tt {\bf compile}([q],t)} & Executes list of queries {\tt q} over the
%specified target {\tt t}.\\
%\hline
%\end{tabular}
%\end{footnotesize}
%\caption{Driver API exposed to \system's Runtime.}
%\label{tab:driver-api} 
%\end{table}
%
%\smartparagraph{Enumerating Partitioning Plans.}
%To enumerate all possible partitioning plans for a given query, \system's runtime 
%considers the different dataflow operators that make up the query and generates 
%partitioned sub-queries for the data plane by incrementally adding one operator 
%at a time. For each sub-query, it uses the {\tt isSupported()} function (see 
%Table~\ref{tab:driver-api}) to ask the driver for the data plane target to check if 
%it can execute the sub-query. It stops when a partitioned sub-query cannot be 
%executed in the data plane. 
%
%To illustrate, consider the case of Query~\ref{asymm-query}. It requires extracting 
%the {\tt dstIP}, {\tt srcIP}, and {\tt proto} fields from the packets and applying the
%dataflow operations {\tt map}, {\tt reduce}, {\tt distinct}, and {\tt filter} over 
%the packet stream. 
%%In this case, the runtime will enumerate eight different sub-queries, 
%%incrementally adding one additional operator for each sub-query. It will then call 
%%the {\tt isSupported()} function in sequence for each of these partitioned sub-queries. 
%PISA targets can execute all the dataflow operations for Query~\ref{asymm-query} 
%in the data plane, and as a result, they can support all the enumerated sub-queries. 
%%
%%For fixed-function data plane targets, the enumeration process will stop after the
%%second sub-query because such targets can only support sub-queries that have only
%%the {\tt filter} operator in Query~\ref{asymm-query}. On the other hand, PISA 
%%switches support both programmable parsing to enable the {\tt map} operations and 
%%state management and user-defined hashing to enable the {\tt reduce} and {\tt distinct} 
%%operations. Thus, 
%%\rjh{In the new structure, this PISA stuff comes out of nowhere.  I don't have a suggestion 
%%for how to fix that right now.}
%To contrast, consider next the case of Query~\ref{payload-query}. It
%requires parsing a packet's payload along with other header fields. Since most
%data plane targets cannot extract these fields in the dataplane, only a small
%set of sub-queries can be enumerated for Query~\ref{payload-query}.
%
%
%\smartparagraph{Selecting Partitioning Plan}
%As the cost $N$ monotonically decreases, and the cost $B$ increases, as we 
%execute more dataflow operations in the data plane. Thus, runtime can greedily
%select the partitioning plan where $N$ is minimum and $B < 1$, \ie~it 
%greedily selects the sub-query with the maximum number of dataflow operators 
%(min $N$) that can be supported by the data plane target($B \le 1$). 
%\system’s runtime asks the driver of  the data plane target to use the {\tt getCost()} 
%function (see Table~\ref{tab:driver-api}) to estimate the cost of executing the sub-query 
%in the data plane.
%
%\subsection{Iterative Refinement}
%\label{ssec:ir}
%
%\begin{figure*}[ht] 
%\begin{minipage}{1\linewidth}
%\begin{subfigure}[b]{.45\columnwidth}
%\includegraphics[trim=0 380 600 0,clip,width=.9\linewidth]{drawings/single_query_ir.pdf}
%\caption{Applying the refinement plan [{\tt dstIP/8, dIP/32}] for 
%Query~\ref{asymm-query}.} 
%\label{fig-single-ir}
%\end{subfigure}
%\begin{subfigure}[b]{.5\columnwidth}
%\lstset{belowskip=0pt}
%\begin{lstlisting}[language=Python,basicstyle=\footnotesize,  escapechar=@,
%basicstyle=\footnotesize, 
%numbers=left,xleftmargin=1em,frame=single,framexleftmargin=2.0em, xrightmargin=1.5em]
%Q1(t) = pktStream(W)
%    .filter(p => p.proto==17)
%\end{lstlisting}
%\lstset{aboveskip=2pt}
%\begin{lstlisting}[numbers=left,xleftmargin=1em,frame=single,framexleftmargin=2.0em, xrightmargin=1.5em, language=Python,basicstyle=\footnotesize,escapechar=@, numbers=left, firstnumber=last, backgroundcolor=\color{yellow}]
%    .filter(p => (p.dstIP/8 in Q1_8(t-W)))
%\end{lstlisting}
%\lstset{belowskip=\medskipamount}
%\begin{lstlisting}[numbers=left,xleftmargin=1em,frame=single,framexleftmargin=2.0em, xrightmargin=1.5em, language=Python,basicstyle=\footnotesize,escapechar=@,
%captionpos=b, firstnumber=last]
%    .map(p => (p.dstIP, p.srcIP))
%    ...
%    .map(p => (dstIP))  
%\end{lstlisting}
%\lstset{aboveskip=\medskipamount}
%\caption{Refined query for Query~\ref{asymm-query}---filtering out the traffic that didn't satisfy the
%query at coarser level of granularity for the previous window interval ($W$).}
%\label{q32}
%\end{subfigure}
%\end{minipage}
%\caption{Iterative refinement in action: (a)~shows how output of coarser query is served as 
%input (as {\tt filter}) for the refined query for the next window interval, (b)~shows how 
%runtime transforms the input query to generate refined queries.} 
%\label{fig:ir} 
%\end{figure*}
%
%%\smartparagraph{Why do we need Iterative Refinement?}
%
%
%\smartparagraph{Enumerating Refinement Plans.}
%Iterative refinement requires a refinement plan. The enumeration of the possible
%refinement plans is performed by applying the following three steps. First, we
%have to determine the fields that can be used for iterative refinement. Next, we
%have to specify the refinement levels for these fields. The third and last step 
%consists of generating all possible refinement plans, \ie~combinations of refinement 
%levels from coarser to finer levels. 
%
%Refinement levels for different fields are configured at boot-time using 
%domain-specific knowledge of the network operators. For example, header 
%fields like {\tt dstIP}, {\tt srcIP} etc. can naturally be refined at the 
%granularity of one bit per iteration, resulting in 32 potential refinement 
%levels for these fields that conform to the IPv4 address format. Other
%fields like {\tt dns.qname} can be similarly refined at the granularity of 
%domain levels. 
%
%Candidate fields for iterative refinement are  determined by identifying the set of 
%fields that (1)~are used as keys in stateful dataflow operations like {\tt reduce}, 
%{\tt filter} etc. and (2)~have a hierarchical structure so as to be replaceable by 
%their coarser versions without missing any traffic that satisfies the original query. 
%\system's runtime checks for the latter requirement by running the query at 
%coarser levels of refinement over representative training data. 
%For example, in the case of Query~\ref{asymm-query}, both {\tt dstIP} and {\tt srcIP} 
%have hierarchical structure and are used as keys in the {\tt distinct} operation, 
%but only {\tt srcIP} can be replaced with its coarser version without missing the 
%traffic that satisfies the original query. While it is possible to have more 
%than one candidate field for iterative refinement, it is also possible to not find 
%any candidate for refinement for a query. Consider the example of 
%the query for detecting sidejacking attacks~\cite{chimera}. This 
%query cannot benefit from iterative refinement because the two
%fields {\tt sessionID} and {\tt userAgent} that are used in the {\tt distinct} 
%operation do not have a hierarchical structure. 
%
%Finally, for generating all possible refinement plans, we consider all possible 
%combinations of refinement levels under the constraint that only refinement steps
%from coarser to finer refinement levels are permitted. For Query~\ref{asymm-query}, 
%there are 32 refinement levels that result in a total of $O(32^3)$ different 
%refinement plans. To illustrate, consider one of these plans, namely the plan 
%{\tt dstIP/8} $\rightarrow$ {\tt dIP/32}. In this case, the input query is first 
%executed at refinement level {\tt dstIP/8}. Then the refinement level {\tt dIP/32} 
%is applied only over the portion of traffic that satisfies the query at {\tt dstIP/8}. 
%Figure~\ref{fig-single-ir} shows the execution of this example refinement plan
%and Figure~\ref{q32} depicts how the query for the {\tt dstIP/32} refinement level 
%is generated for this plan. Here, line 3 ensures that in the current window interval,
%this query is only applied over traffic that satisfied the query at refinement 
%level {\tt dstIP/8} in the previous window interval; that is, the input to this query 
%for the current window interval is the output of the query applied to the previous 
%window interval.
%
%To generate queries for different refinement plans, \system’s runtime has to 
%select appropriate thresholds for queries that get executed at coarser levels. 
%It has to chose these thresholds such that no traffic that satisfies the query 
%at finest level is missed. A strawman solution for threshold selection is to 
%use the network operator-provided threshold that is part of the input query. 
%This choice ensures that executing queries at coarser refinement levels will 
%not miss any traffic of interest. At the same time, such a conservative threshold 
%selection renders iterative refinement largely ineffective for saving compute 
%resources and thus reducing costs, mainly because with such low thresholds, it
%is not possible to effectively filter out the uninteresting traffic at
%the coarser levels. Moreover, since counters for different queries under 
%different workloads scale differently, a solution that uses a fixed scaling factor
%to scale threshold values linearly for coarser refinement levels is also untenable. 
%
%Our solution of this problem relies on representative training data to let the 
%runtime determine appropriate threshold values for each refinement level. 
%In effect, runtime first runs the query at the finest refinement level over the 
%training data to identify the portion of traffic that satisfies the input query. 
%It then executes the query at coarser refinement levels (without applying
%the final {\tt filter} operator) over the portion of traffic that satisfied 
%the input query. Finally, it selects the minimum count from the output which
%ensures that it selects a threshold greater than or equal to the original 
%threshold without missing any traffic that satisfies the query at the coarser 
%refinement levels. For example, for the refinement plan 
%{\tt dstIP/8} $\rightarrow$ {\tt dIP/32}, the runtime finds the threshold for 
%the {\tt dstIP/8} level by executing 
%$Th_{8}$={\tt min(Q(32).map(lambda p: p.dstIP -> dIP/8).join(Q'(8).collect())}.
%Here, {\tt Q} represents the input query and {\tt Q'} is the input query without
%the final {\tt filter} operator.
%
%\smartparagraph{Selecting Refinement Plan.}
%After enumerating candidate refinement plans, the next step is to select the one
%that requires minimum cost. For each refinement level, it greedily executes as 
%many dataflow operators as possible in the data plane---ensuring that stream 
%processor receives as less packets to process as possible; and then selects the
%refinement plan that requires minimum state ($B$) in the data plane. 
%
%However, such a greedy approach does not guarantees best utilization of available 
%resources. For example, for a system configuration where $B_{max}$ is very small 
%compared to $N_{max}$, then greedily selecting the partitioning plan for each 
%refinement level might not return a feasible solution. However, selecting a partitioning 
%plan that selects different partitioning plans for different refinement levels might find 
%feasible solution striking the right balance
%between the two cost metrics. In the next section, we will describe how runtime
%enumerates query plans, \ie~sequence of combination of refinement levels and 
%partitioning plan for each level, and selects the one that finds the minimum cost 
%plan that satisfies system's constraints. 





%\smartparagraph{Execution Costs.}
%We will now reason about the cost of executing dataflow operators. 



%\smartparagraph{Stateful Dataflow Operators.} 
%Line 5 in Query~\ref{dp-query} emits packets with unique {\tt dstIP, srcIP} fields
%in packets' metadata. 
%
%The {\tt reduce} operator can also be executed in 
%similar fashion---requiring changes to the {\tt do\_update}() action only. 
%More generally, executing stateful dataflow operators in the data plane 
%requires (1)~state management primitives, (2)~user-defined hash functions, 
%and (3)~flexible match/action tables. As a result, stateful dataflow operations
%can only be supported by PISA targets in the data plane. 
%
%The data plane driver is responsible for estimating the hash table size for each 
%stateful operator. 
%
%%\mcnote{This sounds unintuitive. Hash tables, a lossless data structure, cannot 
%%meet the error bounds but lossy structures can?}
%%\ag{For same size sketches the error bounds for hash tables are loose.}
%Moreover, as discussed earlier, \system lets network operators specify
%the error bounds for their queries, \ie~probability that packets that satisfy 
%the query are of missed. However, it is not possible to guarantee these error 
%bounds with such simple hash-based implementations. To overcome this problem, 
%the data plane driver leverages sketch-based data structures. For example, in
%the case of the {\tt distinct} operator, the data plane driver relies on
%{\em bloom-filters} to guarantee the specified error bounds. Moreover,
%{\tt reduce} operators with simpler transformation functions (\eg~{\tt sum()}) 
%are implemented as {\em count-min} sketches in the data plane. 

